Federated Learning in IoT: a Survey from a Resource-Constrained Perspective

The IoT ecosystem is able to leverage vast amounts of data for intelligent decision-making. Federated Learning (FL), a decentralized machine learning technique, is widely used to collect and train machine learning models from a variety of distributed data sources. Both IoT and FL systems can be complementary and used together. However, the resource-constrained nature of IoT devices prevents the widescale deployment FL in the real world. This research paper presents a comprehensive survey of the challenges and solutions associated with implementing Federated Learning (FL) in resource-constrained Internet of Things (IoT) environments, viewed from 2 levels, client and server. We focus on solutions regarding limited client resources, presence of heterogeneous client data, server capacity, and high communication costs, and assess their effectiveness in various scenarios. Furthermore, we categorize the solutions based on the location of their application, i.e., the IoT client, and the FL server. In addition to a comprehensive review of existing research and potential future directions, this paper also presents new evaluation metrics that would allow researchers to evaluate their solutions on resource-constrained IoT devices.

==> commmunication.tex <==
\section{Mitigating Communication Overhead}
\label{sec:compress}



==> compiler.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.3\textwidth]{fusion.png}
\caption{Right: unfused convolutional operation that is commonly used in DNNs. Left: Fused kernel that performs the same operation with a single instruction.}
\label{fig:fusion}
\vspace{-0.1in}
\end{figure}

\section{Compiler and Graph Optimizations}


While executing a DNN on any deep learning framework, often similar computations are performed routinely. Researchers have proposed deep learning compilers like TensorRT and XLA that can identify common patterns and optimize them. These complier optimizations include techniques like layer and tensor fusions~\cite{snider2023operator}, kernel tuning~\cite{10.1145/3508391}, and focused convolutions~\cite{tung2022irrelevant}.




In layer fusion techniques, different operations are performed with a single instruction. Layer fusion is depicted in Fig.~\ref{fig:fusion} where the convolution, batch norm, and ReLU operations are fused into a single kernel~\cite{snider2023operator}. Fused kernels reduce the overhead associated with reading and writing the intermediate tensor data for each constituent operations. Kernel auto-tuning techniques~\cite{10.1145/3508391} perform automatic hyper-parameter search to identify the most optimal configurations to meet the required accuracy-efficiency tradeoff. These auto-tuned kernels can vary the tensor precision, network sparsity, batch size, and resolution to vary the DNN's performance. Finally, the focused convolutions modify the General Matrix Multiply (GeMM) algorithm to reduce redundant operations~\cite{tung2022irrelevant}. They focused convolution removes rows from the GeMM input matrix that correspond to ``irrelevant'' pixels to avoid performing convolutions on those inputs. Such techniques are particularly useful in situations where the image background (e.g., trees, sky, buildings) are not relevant to the computer vision task.

Most existing compilers are not general enough to fuse or optimize any DNN architecture. They are well suited for some architectures such as MobileNet~\cite{sandler_mobilenetv2_2018} or BERT~\cite{lanalbert}. Future work on deep learning compilers should focus on generality to improve their use. Furthermore, although compilation is an one-time expense, the resources required for compilation can be significant. More work on optimizing the compilation time will help increase their deployability on IoT devices.





==> conclusions.tex <==
\section{Discussion and Conclusion}

\subsection{Summary of Findings}

This section summarizes our findings related to low-power DNN optimizations. Fig.~\ref{fig:survey} plots the accuracy and energy consumption of different techniques when deployed on IoT devices. The baseline techniques without any optimizations are marked with red circles. Efficient architecture designs such as MobileNetV3~\cite{howard_searching_2019} and EfficientNet~\cite{tan_efficientdet_2020} can lower the energy consumption without sacrificing accuracy. Aggressive 1-bit quantization techniques have been proposed in XNORNet~\cite{xnor} and BinaryNet~\cite{BinNet}, however, these techniques suffer from significant accuracy losses. More research is required to understand how these 1-bit techniques can be used without accuracy losses. More finegrained control over the accuracy vs efficiency tradeoff may be possible by combining different types of techniques. However, most combinations have not yet been explored exhaustively and is an open area of research.

% \subsection{Guidelines for Low-Power Computer Vision}

% There is no single technique to build efficient DNNs for computer vision. Most techniques are complementary and can be used together for better energy efficiency. We include some general guidelines to consider for low-power computer vision.

% \begin{enumerate}
%     \item Quantization and reduced parameter precision decrease the model size and the complexity of arithmetic operations significantly, but unfortunately, it is difficult to manually implement quantization in most machine learning libraries. NVIDIA's TensorRT library provides an interface for such optimizations.
%     \item When optimizing large pre-trained DNNs, pruning and model compression are effective options. 
%     \item When training a new DNN from scratch, compressed convolutional filters and matrix factorizations should be used to reduce the model size and computation.
%     \item NAS finds DNNs that are optimized for individual devices with performance guarantees. DNNs with several branches (e.g. Proxyless-NAS, MNasNet, etc.) frequently require expensive kernel launches and synchronizations on GPUs and CPUs.
%     \item Knowledge distillation should be used with small or medium-sized datasets. This is because fewer assumptions on the DNN architectures of the student and the teacher are required, leading to higher accuracy.
% \end{enumerate}

\subsection{Proposed Evaluation Metrics}

Based on our findings, we propose new evaluation metrics for future researchers to test the deployability of their solutions on low-power IoT devices.
Most DNN-based computer vision techniques are evaluated on just accuracy~\cite{he_deep_2016}. In this section, we present some additional metrics that should be used to evaluate future low-power DNN techniques.

\begin{itemize}
\item The memory requirement to process a single image should be reported. Prior research has shown that memory operations require up to $200\times$ more energy than arithmetic operations~\cite{nazemi_nullanet_2018, lpirc}. Techniques that require less memory, or that are more cache-efficient have advantages on IoT devices. The number of parameters is usually a good proxy for the number of memory operations. However, there are some exceptions to this rule. For example, techniques like MobileNet v1 have a small number of parameters but have low arithmetic intensity (i.e., perform few arithmetic operations for every memory operation). In such cases, the technique may perform many memory operations even with a small number of parameters. As another example, techniques deploying quantization may have more parameters, but require fewer bits per parameter. In such cases, researchers should include results on the scaling of energy consumption with different model sizes and quantization formats.
\item The number of operations is another important metric to compare the efficiency of different techniques. Although each arithmetic operation requires little energy~\cite{nazemi_nullanet_2018}, when DNNs perform billions of operations the energy costs add up. Thus fewer operations are more useful when deploying on resource constrained hardware. Research has found that fully-connected layers require fewer operations than convolutional layers~\cite{simonyan_very_2015}. However, fully-connected layers have more parameters and may require more memory. When designing low-power DNNs, it is important to consider the advantages and disadvantages of the layers based on the available hardware. In most cases, it is important to measure the energy consumption to understand the impact of design decisions.
\end{itemize}

\subsection{Conclusion}

DNNs have gained popularity over the last decade. More recently, their use has become more ubiquitous, and have started to get deployed on low-power IoT devices. However, since most DNNs are designed for high accuracy on server-grade hardware, it is difficult for practitioners to deploy them on battery-powered devices. In this survey, we highlight and summarize the key research topics that help reduce the energy consumption of DNNs so that they can be deployed on IoT devices. We identify that the existing research can be divided into three main categories: (1) neural network compression, (2) network architecture search and design, and (3) compiler and graph optimizations. These techniques have their advantages and disadvantages. We highlight these features and provide recommendations on how these techniques can be improved with continued research.

==> design.tex <==
\section{Architecture Search and Design}
\label{sec:design}


The standard convolution operation is implemented as a tensor multiplication between the parameter tensor and the input tensor.
The same convolution kernel is strided over the entire image to generate the output. Therefore, the number of arithmetic operations performed during convolution is quadratic with the size of the convolution kernel. This knowledge is the motivating reason for many novel DNN architecture designs that use small convolutional kernels. 
The two most famous architectures that use small convolutional kernels are MobileNet~\cite{sandler_mobilenetv2_2018} and SqueezeNet~\cite{iandola_squeezenet_2016}. These DNNs use a new operation called the depthwise separable convolutions to beat the state-of-the-art low-power computer vision solutions. The depthwise separable convolution breaks up a single convolutional kernel into two sub-tasks: (1)~depthwise convolution: applies a single convolutional channel filter on each channel of the input, and (2)~pointwise convolution: performs $1 \times 1$ convolutions to combine the depthwise convolutions. Fig.~\ref{fig:design} shows the benefit of using MobileNet and SqueezeNet over existing DNN architectures. These techniques are can also be used with the previously described pruning and quantization techniques to further increase the efficiency. 
 
\begin{figure}[t!]
\centering
\includegraphics[width=0.49\textwidth]{design.png}
\caption{Comparison of the normalized FLOPs, \#parameters, and accuracy between four representative DNN architectures. MobileNet and SqueezeNet maintain classification accuracy but only require a fraction of the computational resources.}
\vspace{-0.1in}
\label{fig:design}
\end{figure}

EfficientNet and EfficientDet~\cite{tan_efficientdet_2020} provide guidebooks for building different DNN architectures. They showcase the optimal methods to perform layer scaling, width scaling, and resolution scaling. These guides enable the design of compact and accurate DNNs for different resource budgets.

Because there are many different DNN architectures, it can be difficult to select the best DNN for a given task. 
Network Architecture Search (NAS) is a technique that solves this problem by automating architecture selection. NAS uses a ``controller'' to propose DNN architectures. Reinforcement learning is used to evaluate these proposed DNN architectures and then propose another DNN architecture. AmoebaNet~\cite{amoeba} showcases the ability of NAS to obtain state-of-the-art results.


Tan et al.~\cite{MNas} propose MNasNet as a new NAS technique that can build efficient and IoT-friendly DNN models. MNasNet uses two objectives in the reinforcement learning reward function: (1) accuracy and (2) latency.
However, MNasNet requires over 4.6 GPU years to train one DNN architecture for image classification on the ImageNet dataset. This amount of computing resource requirements during training is a challenge that needs to be overcome.


Cai et al.~\cite{proxyless} propose ProxylessNAS, a new NAS technique with the goal of reducing the training overheads.  Proxyless-NAS uses an estimator function to measure the latency and a novel path-level pruning algorithm to reduce the number of candidate architectures. ProxylessNAS reduces the training time of efficient DNNs from 4.6 GPU years to approximately 300 GPU hours. FBNet~\cite{FB} is another technique that reduces the training overheads. FBNet uses a proxy task, i.e., optimizing over a smaller dataset to evaluate candidate architectures. These architecture search techniques are compatible with both convolutional and transformer-based architectures~\cite{liu2022neural}. %https://arxiv.org/pdf/2207.13955.pdf

Future work on architecture search should focus on algorithms that can find architecture designs that contain different building blocks from the existing human-made DNNs. The existing solutions only try different combinations of well-known ``architectural blocks''. Breaking this dependency may allow us to build new architectures.

 


\begin{figure*}[t!]
\centering
\includegraphics[width=0.99\textwidth]{survey.png}
\caption{Comparison of energy consumption and accuracy of different computer vision optimizations. The data-points closer to the bottom right are considered to be the best, i.e., low energy but high accuracy. Circles denote the baseline DNNs deployed without any optimizations. Different techniques can be combined with quantization and pruning to vary the accuracy-efficiency tradeoff. Best viewed in color on a screen.}
\label{fig:survey}
\vspace{-0.1in}
\end{figure*}
